Contextual Stochastic Block Models

We provide the first information theoretic tight analysis for inference of latent community structure given a sparse graph along with high dimensional node covariates, correlated with the same latent communities. Our work bridges recent theoretical breakthroughs in the detection of latent community structure without nodes covariates and a large body of empirical work using diverse heuristics for combining node covariates with graphs for inference. The tightness of our analysis implies in particular, the information theoretical necessity of combining the different sources of information. Our analysis holds for networks of large degrees as well as for a Gaussian version of the model.

==> proofsaux.tex <==
% !TEX root = main.tex
%--------------------------
\section{Proofs of auxiliary lemmas}

==> tools.tex <==
% !TEX root = main.tex
%--------------------------
\section{Useful tools}

We prove some auxiliary lemmas that will be useful in the paper. Some
of the proofs below are known from prior work; we provide references
as well as proofs for completeness.  

\begin{lemma}[{\cite[Proposition 3.1]{talagrand2006free}}]\label{lem:singleFreeEnergy}
Let $g = g_N \in \reals^N$ be a sequence of vectors such that 
$\lim_{N\to\infty}\norm{g}^2/N = a$. Then the following holds:
\begin{align}
\lim_{N\to\infty} \frac{1}{N} \log \E_{\nu_N} \exp(\<g, x\> )
& = \frac{1}{2}\inf_{b \ge 1} \frac{a}{b} + b - 1 - \log b. 
\end{align}
Here $\nu_N$ is the normalized Haar measure on $\sphere^N$. 
\end{lemma}

The following is a similar lemma, for coupled free energies. In this case
we are only interested in an upper bound. 

\begin{lemma}[{\cite[Lemma 7.1]{talagrand2006free}}] \label{lem:coupledFreeEnergy}
Let $(g^1, g^2) = (g^1_N, g^2_N) \in\reals^N \times \reals^N$
be a sequence of vectors so that
\begin{align}
\lim_{N\to\infty} \frac{\norm{g^1}^2}{N} &= a_1, \\
\lim_{N\to\infty} \frac{\norm{g^2}^2}{N} &= a_2, \\
\lim_{N\to\infty} \frac{\<g^1, g^2\>}{N} &= a_c.
\end{align}
Then the following holds for any $b \ge 1$ and $-b\le \kappa \le b$.
\begin{align}
\limsup_{N\to\infty} \frac{1}{N} \log \E_{\nu_N^{\otimes 2}} \exp(\<g^1, x^1\> + \<g^2, x^2\> + \kappa \<x^1, x^2\>  ) 
& \le \frac{a_1+a_2 + 2a_c}{4(b - \kappa)} + \frac{a_1 + a_2 - 2a_c}{4(b + \kappa)} \nonumber \\
&\quad+ b - 1 - \log b
- \log (1- \kappa^2/b^2)
\end{align}
\end{lemma}

We include the classical Slepian inequality below. 
\begin{lemma}[Slepian \cite{vitale2000some}] \label{lem:slepian} Let $A$ be a compact
set in $\reals^N$ and $(X_a)_{a\in A}, (Y_a)_{a\in A}$ be two Gaussian
processes satisfying:
\begin{align}
\E\{(X_a - X_b)^2\} &\le \E\{(Y_a - Y_b)^2\}, \text{ for all } (a, b) \in A\times A. \label{eq:slepiancond}
\end{align}
Then $\E\{ \sup_a X_a\} \le \E\{\sup_a Y_a\}$. 
\end{lemma}

The following lemma is a slight extension of \cite[Lemma 1.1]{panchenko2013sherrington}. 

\begin{lemma}[Gaussian integration by parts]\label{lem:gaussIBP}
Let $\Sigma \subset \reals^N$ be a compact set and $\nu$ be a probability
measure on $\Sigma$. Further, let $X(\sigma)$ and $Y(\sigma)$ be two
jointly Gaussian processes on $\Sigma$. Define the (random) measure $\nu_Y$
on $\Sigma$.
\begin{align}
\d\nu_Y &= \frac{\exp(Y(\sigma))}{\int \exp(Y(\sigma')) \d\nu(\sigma')} \d\nu. 
\end{align}
Let $\Gamma(\sigma^1, \sigma^2) = \E\{X(\sigma^1)Y(\sigma^2)\}$. Then we have
\begin{align}
\E\big\{ \E_{\nu_Y}\{ X(\sigma) \} \big\} &= \E \Big\{ \E_{\nu_Y^{\otimes 2}} \big\{\Gamma(\sigma^1, \sigma^1) - \Gamma(\sigma^1, \sigma^2)  \big\} \Big\}. 
\end{align}

\end{lemma}
\begin{proof}[Proof sketch]
Quantize $\Sigma$ and apply \cite[Lemma 1.1]{panchenko2013sherrington} (which requires $\Sigma$ finite). 
Then use dominated convergence to argue the claim. We might require some more conditions on $\Sigma$ for everything
here to make sense. 
\end{proof}


\subsection{Versions with signal and constraints}

We prove versions of Lemmas \ref{lem:singleFreeEnergy} and \ref{lem:coupledFreeEnergy}
with signal and constraints below. Since they are a little more involved, 
we prove the upper and lower bounds separately in Lemma \ref{lem:singlefreenergysignalupper} and Lemma \ref{lem:singlefreeenergysignallower}

\begin{lemma}\label{lem:singlefreenergysignalupper}
For any vectors $v, g \in \reals^p$, the following holds:
\begin{align}\label{eq:singlefreeenergysignalupper}
 \frac{1}{p} \log \E_{\nu_p} \exp\Big( \frac{1}{2}\<v, x\>^2 + \<g, x\>  \Big) %
 &\le \frac{1}{2} \min_{b \ge 1\vee \norm{v}^2} \frac{\norm{g - g_v}^2}{ pb } + b - 1 - \log b+ \frac{\norm{g_v}^2 }{p (b - \norm{v}^2)} - \frac{1}{p}\log \Big( 1 - \frac{\norm{v}^2}{b}\Big). 
 \end{align} 

\end{lemma}
\begin{proof}
Let $b> 0$ be a parameter and $Y\sim\normal(0, \id_p/b)$. Define $r_p$ by
the following equation:
\begin{align}
\frac{\E\{\norm{Y} \ind( \norm{Y} \ge r_p \sqrt{p}) \}}{\sqrt{p} \P\{\norm{Y}\ge r_p \sqrt{p} \} }& = 1. 
\end{align}
Finally let $\rho \stackrel{d}{=} \norm{Y}/\sqrt{p}$ conditional on
$\norm{Y} \ge r_p\sqrt{p}$. By definition of $r_p$, $\E\{\rho\} = 1$, and
we have that $r_p \le 1$. We can now compute the bound:
\begin{align}
\frac{1}{p} \log \E_{\nu_p} \exp\Big( \frac{1}{2}\<v, x\>^2 + \<g, x\>  \Big)
&= \frac{1}{p} \log \E_{\nu_p} \exp\Big( \frac{\E\{\rho\}^2 }{2}\<v, x\>^2 + \<g, x\> \E\{\rho\} \Big)  \\
&\stackrel{(a)}{\le}  \frac{1}{p} \log \E_{\nu_p} \exp\Big( \frac{\E\{\rho^2\} }{2}\<v, x\>^2 + \<g, x\> \E\{\rho\} \Big)  \\
&\stackrel{(b)}{\le} \frac{1}{p} \log \E  \exp\Big( \frac{1 }{2}\<v, \rho x\>^2 + \<g, \rho x\>  \Big) \\
&\stackrel{(c)}{\le} \frac{1}{p} \log \E  \exp\Big( \frac{1 }{2p}\<v, x \norm{Y}\>^2 + \frac{1}{\sqrt p}\<g, x \norm{Y}\>  \Big) - \frac{1}{p} \log \P\{ \norm{Y} \ge \sqrt{p} r_p \} \\
&\stackrel{(d)}{\le} \frac{1}{p} \log \E  \exp\Big( \frac{1 }{2}\<v, Y\>^2 + \<g, Y\>  \Big) - \frac{1}{p} \log \P\{ \norm{Y} \ge \sqrt{p}  \}.
\label{eq:singlefreeenergysignaluppergaussian}
\end{align}
Here $(a)$ and $(b)$ follow from Jensen's inequality and $(c)$ from the definition
of $\rho$ and removing the conditioning. The step $(d)$ follows from the fact that $\norm{Y}$, $\sqrt{p}\, Y/\norm{Y} \stackrel{d}{=} x$  are
independent, and that  $r_p \le 1$. The right hand side in  \myeqref{eq:singlefreeenergysignaluppergaussian} involves Gaussian integrals, 
which yield for all $b \ge 1 \vee \norm{v}^2$:
\begin{align}
\frac{1}{p} \log \E_{\nu_p} \exp\Big( \frac{1}{2}\<v, x\>^2 + \<g, x\>  \Big)
&\le\frac{1}{2p} \Bigg(\frac{\norm{g - g_v}^2}{b} + \frac{g_v^2}{(b - \norm{v}^2)} +b - 1 - \log b - \log \Big( 1-\frac{\norm{v}^2}{b}\Big )\Bigg).
\end{align}
This completes the lemma.
\end{proof}


\begin{lemma}\label{lem:singlefreeenergyupperminimizer}
Fix any $\eps > 0$. Let $v, g$ be (a sequence of) vectors in $\reals^p$ 
so that $\norm{v}^2$, $\norm{g}^2/p$ and $g_v/\log p$ are
uniformly bounded in $p$. Here $g_v = \<g, v\>/\norm{v}$ is the projection of $g$ 
along $v$.  Define $b_0 = b_0(g, v)$ and $\Delta_0(g, v)$ as follows:
 \begin{align}
 b_0 & = \frac{1}{2} + \sqrt{\frac{1}{4} + \frac{\norm{g-g_v}^2}{p}},\\
 \Delta_0 & = \norm{g_v}\Big( 1-\frac{\norm{g - g_v}^2}{p \norm{v}^2}  - \frac{1}{\norm{v}^2} \Big)^{1/2}
 \end{align}
The following choice of $b_*= b_*(g, v)$ is the minimizer in
Lemma \ref{lem:singlefreenergysignalupper} up to error
$o(p^{-1/2})$: 
 \begin{align}
 b_* &= \begin{cases}
 b_0 , &\text{ if } \norm{g- g_v}^2  \ge p(1+\eps)\norm{v}^4,\\
 \norm{v}^2 + {\Delta_0}/{\sqrt{p}}, &\text{ if } \norm{g- g_v}^2  \le p (1-\eps) \norm{v}^4.
 \end{cases}
 \end{align}

\end{lemma}
\begin{proof}
First we consider the case that $\norm{g - g_v}^2 \ge p (1+\eps) \norm{v}^4$
where $b_* = b_0$.
It is easy to verify that $b_0$ minimizes the following function:
\begin{align}
\frac{1}{2} \Big(\frac{\norm{g - g_v}^2}{pb} + b - 1 - \log b  \Big).
\end{align}
Further, in this case, we see that
\begin{align*}
b_0 - \norm{v^2} & \ge \sqrt{ \frac{\norm{g - g_v}^2}{p} } - \norm{v}^2
\ge \norm{v}^2 (\sqrt{1+\eps} - 1) \ge \norm{v}^2 \eps/ 4.
\end{align*}
Therefore, 
the remaining terms in the upper bound
are $o(p^{-1/2})$ if $\norm{v}^2$ is bounded away from 0. 


Now we consider the case that $\norm{g - g_v}^2 \le p(1-\eps) \norm{v}^2$.
\end{proof}

\begin{lemma}\label{lem:singlefreeenergysignallower}
Let $v, g$ be (a sequence of) vectors in $\reals^p$ 
so that $\norm{v}^2$, $\norm{g}^2/p$ 
and $g_v/\log p$ are
uniformly bounded in $p$. Then the bound of 
Lemma \ref{lem:singlefreenergysignalupper} is tight
up to $o(p^{-1/2})$ errors, i.e. 
\begin{align}
\frac{1}{p} \log \E_{\nu_p} \exp\Big( \frac{1}{2}\<v, x\>^2 + \<g, x\>  \Big) %
 &\ge \frac{1}{2}  \frac{\norm{g - g_v}^2}{ pb_* } + b_* - 1 - \log b_*+ \frac{\norm{g_v}^2 }{p (b_* - \norm{v}^2)} - \frac{1}{p}\log \Big( 1 - \frac{\norm{v}^2}{b_*}\Big) + o(p^{-1/2}).
\end{align}
\end{lemma}
\begin{proof}



For the lower bound, for any fixed $u_1, u_2 \in [0, 1]$, we have:
\begin{align}
\frac{1}{p}\log \E_{\nu_p} \exp\Big( \frac{1}{2}\<v, x\>^2 + \<g, x\>  \Big) 
& \ge \frac{1}{p} \Big(  \frac{p \norm{v}^2 u_1}{2} + {g_v \sqrt{ pu_1}} + \norm{g - g_v}\sqrt{p u_2} \Big)  \nonumber\\ 
&\quad+ \frac{1}{p} \log \P_{\nu_p}\big\{ \<v, x\> \ge \norm{v}\sqrt{p u_1}, \<g - g_v, x\> \ge \norm{g - g_v} \sqrt{p u_2} \big\} \\
&=   \frac{ \norm{v}^2 u_1}{2} + g_v \sqrt\frac{u_1}{p}+ \norm{g - g_v}\sqrt{\frac{u_2}{p}} \Big)  \nonumber\\ 
&\quad+ \frac{1}{p} \log \P_{\nu_p}\big\{ x_1 \ge \sqrt{p u_1}, x_2 \ge  \sqrt{p u_2} \big\} \label{eq:userotinv} \\
&= \frac{\norm{v}^2u_1}{2} + \norm{g - g_v}\sqrt\frac{u_2}{p} -\frac{1}{2}\log( 1- u_1 - u_2) + O\Big(\frac{\log p}{p}\Big),
\end{align}
where \myeqref{eq:userotinv} follows 
by the rotational invariance of $\nu_p$ and the final line is a classical
large deviations estimate. At this stage, we consider two cases
corresponding to the two cases in Lemma \ref{lem:singlefreeenergyupperminimizer}.

\end{proof}



